Foundations of Symbolic Languages for Model Interpretability

Several queries and scores have recently been proposed to explain individual predictions over ML models. Given the need for flexible, reliable, and easy-to-apply interpretability methods for ML models, we foresee the need for developing declarative languages to naturally specify different explainability queries. We do this in a principled way by rooting such a language in a logic, called FOIL, that allows for expressing many simple but important explainability queries, and might serve as a core for more expressive interpretability languages. We study the computational complexity of FOIL queries over two classes of ML models often deemed to be easily interpretable: decision trees and OBDDs. Since the number of possible inputs for an ML model is exponential in its dimension, the tractability of the FOIL evaluation problem is delicate but can be achieved by either restricting the structure of the models or the fragment of FOIL being evaluated. We also present a prototype implementation of FOIL wrapped in a high-level declarative language and perform experiments showing that such a language can be used in practice.

==> decision-tree-bias.tex <==
\centering
\scalebox{0.8}{
\begin{tikzpicture}
	\node at (-3.5, 3) (vn) {\small $\begin{matrix}
	   	\text{Stable job}\\
	   	>\text{ 40yo}\\
	   	\text{Previous loans}\\
	   	\text{Owns a house}\\
	  	\text{Has kids}\\
	  	\text{Married}\\
	  	\text{Criminal Record}
	   \end{matrix}$};

	\node at (-1.5, 3) (v) {$\begin{pmatrix}
	   	1\\
	   	1\\
	   	1\\
	   	0\\
	   	0\\
	  	1\\
	  	0
	   \end{pmatrix}$};
	   
	\node at (-0.6, 3) (v2) {$\begin{pmatrix}
	   	1\\
	   	1\\
	   	1\\
	   	0\\
	   	0\\
	  	1\\
	  	1
	   \end{pmatrix}$};

	   
	\node at (-1.5, 4.7) {$\vx$};
	\node at (-0.6, 4.7) {$\vy$};



\node (wm) at (4,6) {{\bf Stable Job}};
    \node (oc1) at (2,4.5) {{\bf Has kids}};
        \node (f1) at (1,3) {$\false$};
        \node (ft1) at (3,3) {\underline{{\bf Married}}};
            \node (t1) at (0.5, 1.5) {$\true$};
            \node (ak) at (4,1.5) {{\bf Owns a house}};
            \node (ak2) at (9.5,3) {{\bf Previous Loans}};
            	    \node (f0) at (2, 1.5) {$\false$};	           
                \node (f3) at (3,0) {$\false$};
                \node (t2) at (5,0) {$\true$};
                	\node (f4) at (7,0) {$\false$};
                	
                	\node (t3) at (10,1.5) {$\true$};
                	\node (f5) at (8,1.5) {$\false$};
    \node (ft2) at (6,4.5) {\underline{{\bf Criminal Record}}};
        \node (oc2) at (5.5,3) {{\bf Previous Loans}};


\draw[black, thick,->] (wm) -- (oc1) node[pos=0.6, above] {$0$};
\draw[black, thick,->] (oc1) -- (f1) node[midway,left] {$1$};
\draw[black, thick,->] (oc1) -- (ft1) node[midway,right] {$0$};
\draw[black, thick,->] (ft1) -- (t1) node[midway,left] {$0$};
\draw[black, thick,->] (ft1) -- (f0) node[midway,right] {$1$};
\draw[red,  ultra thick,->] (ak) -- (f3) node[midway,left] {$0$};
\draw[black, thick,->] (ak) -- (t2) node[midway,right] {$1$};

\draw[blue, ultra thick,->] (wm) -- (ft2) node[pos=0.5, above] {$1$};
\draw[blue, ultra thick,->] (ft2) -- (ak2) node[pos=0.3, below] {$0$};
\draw[red, ultra thick,->] (ft2) -- (oc2) node[midway,right] {$1$};
\draw[black, thick,->] (oc2) -- (f4) node[midway,right] {$0$};
\draw[red, ultra thick,->] (oc2) -- (ak) node[midway,left,above] {$1$};

\draw[blue, ultra thick,->] (ak2) -- (t3) node[midway,right] {$1$};
\draw[black, thick,->] (ak2) -- (f5) node[midway,left] {$0$};
\end{tikzpicture}
}

==> fragments.tex <==
%%%%%%%%%%%%%%%%%%%%%
%Rough ideas:
%  - We know that there are several tractability/intractability results for models 
%  - We show here that several of them can be obtained as a consequence of general results for our logical language
%%%%%%%%%%%%%%%%%%%%%

\todo[inline]{We should put the most general and uniform fragment for which we have a tractability result.}
\begin{theorem}
\label{theo:alg-positive}
Every query in \foil$(F)$ can de evaluated in polynomial time over Decision Trees. 
\end{theorem}

\begin{corollary}
All the following explainability tests can be evaluated in polynomial time over Decision Trees.
\begin{enumerate}
	\item
	\item
\end{enumerate}
\end{corollary}



==> introduction.tex <==



**********************************************

\begin{itemize}
\item It seems that "model Interpretability" is mainly about "our ability to understand models", either globally or locally. Therefore, the degree of interpretability of a model is intimately related with our ability to "answer questions" about it. Those questions can either be global questions (behavior of the model as a whole) or local questions (its behavior regarding certain instances/features).

\item One can find claims in the literature about classes of models like DNF, or Rule Lists, being interpretable. Even though they can be convincing on small examples, there are many important questions we cannot answer about said models. For example, whether they accept all inputs or not (coNP-hard). 

\item It is thus relevant to attempt to better specify which kind of questions we should be able to answer about models in order to claim that they are interpretable and we  can understand them. 

\item We can say that a "local" question about a model is one that has some (partial) instances as input (they will be our free variables) and a "global" question is one that has none, it only depends on the model itself.

\item It is natural to say that, if Q is a question (local or global) that we want to be able to answer for interpretable models, then we should also be able to answer ~Q. Similarly for P, Q and then P v Q, P \& Q. If Q(x,y, z, ...) is a local question, it seems natural that Exists x, Q(x,y,z, ...) is also a reasonable interpretability question, and so on.

\item This naturally motivates a First Order language. We argue that Positive and Subsumption are the minimum elements such a language would need to include: Positive is obvious, and Subsumption comes from the fact that we want to be able to reason about instances that share features or are related in some way.

\item We present a logical structure with only those two predicates, and show that just those two are enough to express many interesting interpretability queries.

\item We present how on top of such a logical structure one could build a query language with an intuitive and high-level syntax, that could actually be used by practitioners.

\item We study the complexity of evaluating this logic, and find out that it is usually very hard to do so. Moreover, it provides arguable evidence that models as simple as Decision Trees are not entirely interpretable, by giving insight into natural queries that are not easy to answer over them.

\item We find a restrictive class of models for which every query in the logic is easy to evaluate, and also prove some sufficient conditions for classes of models that would have the same result.

\item (Maybe) We study fragments of the logic that are tractable over classes of models (Monotone-DNF, Decision Trees, Perceptrons, etc.). The existential fragment is usually much easier to deal with.

\item We implemented a compiler high-level-syntax -> logic, and a solver for a fragment of the logic for FBDDs, and show how to use it for Decision Trees with numeric features (i.e., not necessarily boolean). Queries with few variables/connectives (which are probably the kind that will written in practice), work very fast (under 10milliseconds).
\end{itemize}

==> models.tex <==
\begin{proposition}
There exists a query $\varphi$ in \foil\ such that evaluating $\varphi$ over Decision Trees is NP-hard.
\end{proposition}

\todo[inline]{Here we should talk about the naturality of the query, which interpretability problem it defines and the implication that explaining Decision Trees is not always easy.}

\subsection*{Restricting models to obatin general tractability}

\begin{theorem}
Every query in \foil\ can be evaluated in polynomial time over Bounded Decision Trees.
\end{theorem}

\begin{theorem}
Every query in \foil\ can be evaluated in polynomial time over Decision Rules.
\end{theorem}

==> monoton-dnf.tex <==
\section{Monotone DNF formulas}

\newcommand{\N}{{\cal N}}
\newcommand{\U}{{\cal U}}  
\newcommand{\D}{{\cal D}}

We show that the FO-evaluation over monotone DNF formulas is NP-hard. 
%\newcommand{\P}{{\cal P}} 
Before starting we define several important \FO-formulas over the vocabulary containing only the relation symbol $\subseteq$.
We use $\bar u,\bar v,\bar w,\dots$ to denote variables used by such formulas and which are interpreted over tuples in $\{0,1,\bot\}^t$, for some $t > 0$. 
%If $\bar a \in \{0,1,\bot\}^t$ and $a_i \in \{0,1\}$, then we say that the $i$-th component of $\bar a$ is {\em defined}. 
\begin{itemize}
\item ${\sf Bottom}(\bar u) := \neg \exists \bar v (\bar v \subset \bar u)$. That is, ${\sf Bottom}$ defines the set that only consists of the tuple $\{\bot\}^{t}$ in which all components are unknown. 
\item ${\sf Full}(\bar u) := \neg \exists \bar v (\bar u \subset \bar v)$. That is, ${\sf Full}$ defines the set that only consists of tuple in $\{0,1\}^{t}$.
%\item ${\sf Single}(\bar u) := \forall \bar v (\bar v \subset \bar u \, \rightarrow \, {\sf Undef}(\bar v))$. 
%That is, ${\sf Single}$ defines the set that consists precisely of those tuples in 
%$\{0,1,\bot\}^{t}$ which have at most one component that is defined. 
%\item ${\sf Full}(\bar u) := \neg \exists \bar v (\bar u \subset \bar v)$. That is, ${\sf Full}$ defines the set of tuples in $\{0,1\}^t$; i.e, those tuples without undefined components. 
%\item $(\bar u \sqcup \bar v = \bar z) := (\bar u \subseteq \bar z) \wedge (\bar v \subseteq \bar z) \wedge \neg \exists \bar w \big((\bar u \subseteq \bar z) \wedge (\bar v \subseteq \bar z) \wedge (\bar z \subset \bar w)\big)$. That is, $\bar z$, if it exists, is the {\em join} of $\bar u$ and $\bar v$. 
\item $(\bar u \sqcap \bar v = \bar z) := (\bar z \subseteq \bar u) \wedge (\bar z \subseteq \bar v) \wedge \neg \exists \bar w \big((\bar z \subseteq \bar u) \wedge (\bar z \subseteq \bar v) \wedge (\bar w \subset \bar z)\big)$. That is, $\bar z$ is the {\em meet} of $\bar u$ and $\bar v$ (which always exists). 
\item ${\sf Comp}(\bar u,\bar v) := {\sf Full}(\bar u) \wedge {\sf Full}(\bar v) \wedge \forall \bar z \big(\bar u \sqcap \bar v = \bar z \, \rightarrow \, {\sf Undef}(\bar z)\big)$. That is, ${\sf Comp}(\bar u,\bar v)$ holds iff 
$\bar u$ and $\bar v$ are full and $u_i = 1 - v_i$ for each $i \in [0,t]$. 
\item ${\sf dist}_1(\bar u,\bar v) := \bar u \subset \bar v \wedge \neg \exists \bar z (\bar u \subset \bar z \wedge \bar z \subset \bar v)$. 

\end{itemize}
%${\sf Comp}(\bar u,\bar v) := \exists \bar w \exists z ({\sf Undef}(\bar z) \, \wedge \, \bar u \sqcup \bar v = \bar z \, \wedge \, \bar u \sqcap \bar v = \bar w)$.   
%That is, ${\sf Comp}$ defines the pairs $(\bar a,\bar b)$ 
%of tuples in $\{0,1,\bot\}^t \times \{0,1,\bot\}^t$ such that no component that is defined in $\bar a$ is also defined in $\bar b$, and viceversa. In fact, assume 
%for the sake of contradiction that this is not the case. By symmetry, we only have to consider two cases.
%\begin{itemize}
%\item There is an $i \leq t$ with $a_i = 1$ and $b_i = 0$. Then the join of %\bar a$ and $\bar b$ does not exist. 
%\item There is an $i \leq t$ with $a_i  = b_i = 1$. Then the $i$-th component of the meet of $\bar a$ and $\bar b$ is 1, and hence $\bar a \sqcap \bar b = \{\bot\}^t$. 
%\end{itemize} 
%\item ${\sf MaxComp}(\bar u,\bar v) := {\sf Comp}(\bar u,\bar v) \, \wedge \, \neg \exists \bar w \big((\bar v \subseteq \bar w) \wedge {\sf Comp}(\bar u,\bar w)\big)$.    
%That is, ${\sf MaxComp}$ defines the pairs $(\bar a,\bar b)$ such that the components that are defined in $\bar a$ are precisely the ones that are undefined in $\bar b$, and viceversa.  
%Notice, by definition, that if $(\bar a,\bar b)$ belongs to the interpretation of ${\sf MaxComp}$ then $\bar a \sqcup \bar b$ exists 
%and belongs to the interpretation of ${\sf Full}$. 
%\item ${\sf Rel}(\bar u,\bar v) := \neg \exists \bar w \big((\bar w \subseteq \bar v)  \, \wedge \, {\sf Single}(\bar w) \, \wedge\, {\sf Comp}(\bar u,\bar w)\big)$. 
%That is, ${\sf Rel}$ defines the pairs $(\bar a,\bar b)$ 
%of tuples in $\{0,1,\bot\}^t \times \{0,1,\bot\}^t$ such that every component that is defined in $\bar b$ is also defined in $\bar a$.
%\item ${\sf MaxRel}(\bar u,\bar v) := {\sf Rel}(\bar u,\bar v) \, \wedge \, \neg \exists \bar w \big((\bar v \subset \bar w) \wedge {\sf Rel}(\bar u,\bar w)\big)$.    
%That is, ${\sf MaxRel}$ defines the pairs $(\bar a,\bar b)$ such that the components defined in $\bar a$ and in $\bar b$ are the same.  
%Notice, by definition, that if $(\bar a,\bar b)$ belongs to the interpretation of ${\sf MaxComp}$ then $\bar a \sqcup \bar b$ exists 
%and belongs to the interpretation of ${\sf Full}$. 
% 
%\end{itemize}

We now explain the reduction. 
Consider an instance of the following problem, which we know it is {\sc NP}-complete. 
The instance consists of a propositional formula 
$\phi = C_1 \wedge \ldots \wedge C_m$ in 3DNF in which each $C_i$, for $i \leq m$, is a conjunction of exactly three propositional 
variables from a set $\{x_1,\dots,x_n\}$. We want to check if there 
is an assignment $\sigma : \{x_1,\dots,x_n\} \to \{0,1\}$ such that, for each conjunction $C_i$ with $i \leq m$, 
there is exactly one variable in $C_i$ that is assigned value 0 under $\sigma$.   
Consider a full instance $\bar a \in \{0,1\}^t$. Observe that the following holds:
\begin{itemize} 
\item There is a conjunction $C_i$ in $\phi$ whose variables receive value $(1,1,1)$ under the assignment defined by $\bar a$ iff $\astruct_{\phi} \models {\sf AllOne}(\bar a)$, for ${\sf AllOne}(\bar u) = \pos(\bar u)$.
\item There is a conjunction $C_i$ in $\phi$ whose variables receive value $(0,0,0)$ under the assignment defined by $\bar a$ iff $\astruct_{\phi} \models {\sf AllZero}(\bar a)$, for ${\sf AllZero}(\bar u) = \forall \bar v ({\sf Comp}(\bar u,\bar v) \rightarrow {\sf AllOne}(\bar v))$. 
\item There is a conjunction $C_i$ in $\phi$ whose variables receive value $(0,1,1)$, $(1,1,0)$, or $(1,0,1)$ under the assignment defined by $\bar a$ if $\astruct_{\phi} \models {\sf OneZero}(\bar a)$, for  
${\sf OneZero}(\bar u) := 
\exists \bar v ({\sf dist}_1(\bar v,\bar u) \wedge  \exists \bar z ({\sf dist}_1(\bar v,\bar z) \wedge \pos(\bar z))$.
\item There is a conjunction $C_i$ in $\phi$ whose variables receive value $(0,0,1)$, $(1,0,0)$, or $(1,0,1)$ under the assignment defined by $\bar a$ if $\astruct_{\phi} \models {\sf TwoZeros}(\bar a)$, for  
${\sf TwoZeros}(\bar u) := 
\forall \bar v ({\sf Comp}(\bar u,\bar v) \rightarrow {\sf Onezero}(\bar v))$. 
\end{itemize} 

Hence, there 
is an assignment $\sigma : \{x_1,\dots,x_n\} \to \{0,1\}$ such that, for each conjunction $C_i$ with $i \leq m$, 
there is exactly one variable in $C_i$ that is assigned value 0 under $\sigma$, iff $\astruct_\phi \models \psi$, where 
$$\psi \ = \ \exists \bar u \, \big({\sf Full}(\bar u) \, \wedge \, \neg {\sf AllOne}(\bar u) \, \wedge \, \neg {\sf AllZero}(\bar u) \, \wedge \, \neg 
{\sf TwoZeros}(\bar u)\big).$$ 


%We assume, without loss of generality, that $m = 2^q$ for some integer $q > 0$.  

%With each $V \subseteq \{x_1,\dots,x_n\}$, we associate a different tuple %$\bar V \in \{\bot\}^q \times \{0,1\}^n$ defined as %$(\bot,\ldots,\bot,\chi_V)$, where $\chi_V \in \{0,1\}^n$ is the 
%tuple whose $i$-th component is a 1, if $x_i \in V$, and it is a 0 otherwise. 
%Analogously, with each clause $C_j$, for $j \leq m$, we associate a different tuple $\bar C_j \in \{0,1\}^q \times \{\bot\}^n$ defined as $([j-1],\bot,\ldots,\bot)$, 
%where $[j-1] \in \{0,1\}^q$ is the 
%binary encoding of $j-1$. Furthermore, we write $(\bar C_j,\bar V)$ for the instance $([j-1],\chi_V) \in \{0,1\}^{q+n}$. Notice that 
%$\bar C_j \sqcup \bar V = (\bar C_j,\bar V)$. 
%$(\bar x_i,\bar C_j)$ is the only tuple $\bar v \in \{0,1\}^{p+q}$ which satisfies $\bar x_i,\bar C_j \subseteq \bar v$.   

%\subsection{A tractable fragment over Monotone DNF formulas}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> preliminaries.tex <==

\subsection{Decision Trees}
Let~$X$ be a finite set of \emph{features}, also called
\emph{variables}. An \emph{entity} over~$X$ is a function~$\es:X \to
\{0,1\}$. A \emph{binary decision diagram}
(BDD~\cite{wegener2004bdds}) over $X$ is a rooted directed acyclic
graph~$\mathcal{M}$ with labels on edges and nodes such that: (i) each
leaf is labeled with~$\true$ or $\false$; (ii) each internal node (a
node that is not a leaf) is labeled with a feature $x \in X$; and
(iii) each internal node has two outgoing edges, one labeled~$1$ and
the another one labeled~$0$. Every entity $\es$ over $X$ defines a
unique path $\pi_\es = u_1 \cdots u_k$ from the root $u_1$ to a leaf
$u_k$ of $\M$ such that: if the label of
$u_i$ is $x \in X$, where $i \in \{1, \ldots, k-1\}$, then the edge from $u_i$ to $u_{i+1}$ is labeled with $\es(x)$. Moreover, the entity $\es$ is positive, denoted by
$\mathcal{M}(\es) = 1$, if the label of $u_k$
%the leaf in the path $\pi_\es$
is~$\true$; otherwise the entity $\es$ is negative, which is denoted
by $\mathcal{M}(\es) = 0$. The \emph{size}~$|\mathcal{M}|$
of~$\mathcal{M}$ is its number of edges.  A binary decision
diagram~$\mathcal{M}$ is \emph{free} (FBDD) if for every path from the
root to a leaf, no two nodes on that path have the same label. A
\emph{decision tree} is simply an FBDD whose underlying graph is a
tree.



\subsection{First-Order Logic}


==> proof-dt.tex <==
%\newcommand{\P}{{\cal P}} 
\newcommand{\N}{{\cal N}}
\newcommand{\U}{{\cal U}}  
\newcommand{\D}{{\cal D}}

Before starting we define several important \FO-formulas over the vocabulary containing only the relation symbol $\subseteq$.
We use $\bar u,\bar v,\bar w,\dots$ to denote variables used by such formulas and which are interpreted over tuples in $\{0,1,\bot\}^t$, for some $t > 0$. 
If $\bar a \in \{0,1,\bot\}^t$ and $a_i \in \{0,1\}$, then we say that the $i$-th component of $\bar a$ is {\em defined}. 
\begin{itemize}
\item ${\sf Undef}(\bar u) := \neg \exists \bar v (\bar v \subset \bar u)$. That is, ${\sf Undef}$ defines the set that only consists of the tuple $\{\bot\}^{t}$ in which all components are undefined. 
\item ${\sf Single}(\bar u) := \forall \bar v (\bar v \subset \bar u \, \rightarrow \, {\sf Undef}(\bar v))$. 
That is, ${\sf Single}$ defines the set that consists precisely of those tuples in 
$\{0,1,\bot\}^{t}$ which have at most one component that is defined. 
%\item ${\sf Full}(\bar u) := \neg \exists \bar v (\bar u \subset \bar v)$. That is, ${\sf Full}$ defines the set of tuples in $\{0,1\}^t$; i.e, those tuples without undefined components. 
\item $(\bar u \sqcup \bar v = \bar z) := (\bar u \subseteq \bar z) \wedge (\bar v \subseteq \bar z) \wedge \neg \exists \bar w \big((\bar u \subseteq \bar z) \wedge (\bar v \subseteq \bar z) \wedge (\bar z \subset \bar w)\big)$. That is, $\bar z$, if it exists, is the {\em join} of $\bar u$ and $\bar v$. 
\item $(\bar u \sqcap \bar v = \bar z) := (\bar z \subseteq \bar u) \wedge (\bar z \subseteq \bar v) \wedge \neg \exists \bar w \big((\bar z \subseteq \bar u) \wedge (\bar z \subseteq \bar v) \wedge (\bar w \subset \bar z)\big)$. That is, $\bar z$ is the {\em meet} of $\bar u$ and $\bar v$ (which always exists). 
\item ${\sf Comp}(\bar u,\bar v) := \exists \bar w \exists z ({\sf Undef}(\bar z) \, \wedge \, \bar u \sqcup \bar v = \bar z \, \wedge \, \bar u \sqcap \bar v = \bar w)$.   
That is, ${\sf Comp}$ defines the pairs $(\bar a,\bar b)$ 
of tuples in $\{0,1,\bot\}^t \times \{0,1,\bot\}^t$ such that no component that is defined in $\bar a$ is also defined in $\bar b$, and viceversa. In fact, assume 
for the sake of contradiction that this is not the case. By symmetry, we only have to consider two cases.
\begin{itemize}
\item There is an $i \leq t$ with $a_i = 1$ and $b_i = 0$. Then the join of $\bar a$ and $\bar b$ does not exist. 
\item There is an $i \leq t$ with $a_i  = b_i = 1$. Then the $i$-th component of the meet of $\bar a$ and $\bar b$ is 1, and hence $\bar a \sqcap \bar b = \{\bot\}^t$. 
\end{itemize} 
\item ${\sf MaxComp}(\bar u,\bar v) := {\sf Comp}(\bar u,\bar v) \, \wedge \, \neg \exists \bar w \big((\bar v \subseteq \bar w) \wedge {\sf Comp}(\bar u,\bar w)\big)$.    
That is, ${\sf MaxComp}$ defines the pairs $(\bar a,\bar b)$ such that the components that are defined in $\bar a$ are precisely the ones that are undefined in $\bar b$, and viceversa.  
%Notice, by definition, that if $(\bar a,\bar b)$ belongs to the interpretation of ${\sf MaxComp}$ then $\bar a \sqcup \bar b$ exists 
%and belongs to the interpretation of ${\sf Full}$. 
\item ${\sf Rel}(\bar u,\bar v) := \neg \exists \bar w \big((\bar w \subseteq \bar v)  \, \wedge \, {\sf Single}(\bar w) \, \wedge\, {\sf Comp}(\bar u,\bar w)\big)$. 
That is, ${\sf Rel}$ defines the pairs $(\bar a,\bar b)$ 
of tuples in $\{0,1,\bot\}^t \times \{0,1,\bot\}^t$ such that every component that is defined in $\bar b$ is also defined in $\bar a$.
\item ${\sf MaxRel}(\bar u,\bar v) := {\sf Rel}(\bar u,\bar v) \, \wedge \, \neg \exists \bar w \big((\bar v \subset \bar w) \wedge {\sf Rel}(\bar u,\bar w)\big)$.    
That is, ${\sf MaxRel}$ defines the pairs $(\bar a,\bar b)$ such that the components defined in $\bar a$ and in $\bar b$ are the same.  
Notice, by definition, that if $(\bar a,\bar b)$ belongs to the interpretation of ${\sf MaxComp}$ then $\bar a \sqcup \bar b$ exists 
and belongs to the interpretation of ${\sf Full}$. 
% 
\end{itemize}

We now explain the reduction. 
Consider an instance of the problem {\sc Positive One-in-Three 3Sat}, which we know it is {\sc NP}-complete. 
Recall that such an instance consists of a propositional formula 
$\phi = C_1 \wedge \ldots \wedge C_m$ in 3CNF in which each clause $C_i$, for $i \leq m$, is a disjunction of exactly three propositional 
variables from a set $\{x_1,\dots,x_n\}$. We want to check if there 
is an assignment $\sigma : \{x_1,\dots,x_n\} \to \{0,1\}$ such that, for each clause $C_i$ with $i \leq m$, 
there is exactly one variable in $C_i$ that is assigned value 1 under $\sigma$.   
We assume, without loss of generality, that $m = 2^q$ for some integer $q > 0$.  

With each $V \subseteq \{x_1,\dots,x_n\}$, we associate a different tuple $\bar V \in \{\bot\}^q \times \{0,1\}^n$ defined as $(\bot,\ldots,\bot,\chi_V)$, where $\chi_V \in \{0,1\}^n$ is the 
tuple whose $i$-th component is a 1, if $x_i \in V$, and it is a 0 otherwise. 
Analogously, with each clause $C_j$, for $j \leq m$, we associate a different tuple $\bar C_j \in \{0,1\}^q \times \{\bot\}^n$ defined as $([j-1],\bot,\ldots,\bot)$, 
where $[j-1] \in \{0,1\}^q$ is the 
binary encoding of $j-1$. Furthermore, we write $(\bar C_j,\bar V)$ for the instance $([j-1],\chi_V) \in \{0,1\}^{q+n}$. Notice that 
$\bar C_j \sqcup \bar V = (\bar C_j,\bar V)$. 
%$(\bar x_i,\bar C_j)$ is the only tuple $\bar v \in \{0,1\}^{p+q}$ which satisfies $\bar x_i,\bar C_j \subseteq \bar v$.   

From our input instance we build a decision tree $\D_\phi$, of arity $(q+n)$, that accepts precisely the tuples $(\bar C_j,\bar V) \in \{0,1\}^{q+n}$ satisfying that 
$V$ contains exactly 
one propositional variable from $C_j$. 

\begin{claim}
The decision tree $\D_\phi$ can be constructed in polynomial time from our input instance.
\end{claim}

\begin{proof} 
We build a complete decision tree for the first $q$ variables, which is of size $O(m)$ and thus polynomial on the input.  
For each $j \leq m$, we extend the leaf representing $[j-1]$ with a decision tree of depth three which checks if $V$ contains exactly one of the propositional variables in 
$C_j$. This decision tree is defined over the propositional variables in $C_j$. 
As an example, if $C_j = x_1 \wedge x_3 \wedge x_7$, then the decision tree first tests for the value of $x_1$. If $x_1 = 1$, it checks that $x_3 = x_7 = 0$. 
If $x_1 = 0$, it checks if either $x_3 = 1$ or $x_7 = 1$.  
\end{proof}

We now define a \FO\ formula
%\begin{multline*}
$$
\phi(\bar u) \ := \ \exists \bar v \, \bigg( \, {\sf MaxRel}(\bar u,\bar v) \, \wedge \, \forall \bar w \forall \bar z \big({\sf MaxComp}(\bar u,\bar w) \wedge (\bar v \sqcup \bar w = \bar z) \, \rightarrow \, \pos(\bar z) \big) \, \bigg).  
$$
%
%\forall \bar v \bigg( \, {\sf MaxComp}(\bar u,\bar v) \, \rightarrow \, \\ \exists! \bar w 
%\big(\, {\sf MaxRel}(\bar u,\bar w) \wedge \forall \bar z (\bar w \cap \bar u' = \bar z \rightarrow \pos(\bar z)) \, \big) \, \bigg). 
%\end{multline*}

Finally, we prove that our original instance $C_1 \wedge \ldots \wedge C_m$ of {\sc Positive One-in-Three 3Sat} has a solution if, and only if, 
$\astruct_{\D_\phi} \models \phi(\bar X)$, for $X = \{x_1,\dots,x_n\}$. (Recall that $\bar X \in \{\bot\}^q \times \{0,1\}^n$ is the tuple $(\bot,\ldots,\bot,\chi_X)$). 

Assume first that $C_1 \wedge \ldots \wedge C_m$ has a solution. This is an assignment $\sigma : \{x_1,\dots,x_n\} \to \{0,1\}$ that satisfies exactly one variable per clause. 
Let $V$ be the set of all variables in $\{x_1,\dots,x_n\}$ that are assigned value 1 under $\sigma$. 
We show that, in order to satisfy $\phi(\bar X)$ in $\astruct_{\D_\phi}$, 
the existentially quantified variable $\bar v$ can be witnessed by the tuple $\bar V \in \{\bot\}^q \times \{0,1\}^n$. 
In fact, the components which are defined in $\bar V$ and in $\bar X$ are the same, and hence 
$(\bar X,\bar V)$ belongs to the interpretation of ${\sf MaxRel}$. 
%Moreover, the set defined by the formula $\bar a  \subseteq \bar u' \wedge {\sf MaxRel}(\bar x_1,\bar u')$ over $\astruct_{\D_\phi}$ is precisely $\{\bar x_i \mid x_i \in X\}$. 
Now, take an arbitrary tuple $\bar a \in \{0,1,\bot\}^{q+n}$ 
satisfying $\astruct_{\D_\phi} \models {\sf MaxComp}(\bar X,\bar a)$. 
By definition, then, $\bar a \in \{0,1\}^q \times \{\bot\}^n$, and hence $\bar a = \bar C_j$ for some $j \leq m$. 
By hypothesis, 
there exists exactly one propositional variable in $C_j$ receiving value $1$ under $\sigma$. 
Hence, there exists exactly one propositional variable in $C_j$ that belongs to $V$. We conclude that $(\bar C_j \cup \bar V) = (\bar C_j,\bar V)$ belongs to the interpretation of predicate 
$\pos$ in $\astruct_{\D_\phi}$, which implies that $\astruct_{\D_\phi} \models \phi(\bar X)$. 
%
%there is exactly one tuple $\bar x$ in the interpretation of  
%%$\bar a  \subseteq \bar u' \wedge {\sf MaxRel}(\bar x_1,\bar u')$ over $\astruct_{\D_\phi}$ for which it holds that the meet of $\bar x$ and $\bar C_j$ is a positive instance of $\D_\phi$. This tuple $\bar x$ is 
%%precisely $\bar x_i$.

Assume now that $\astruct_{\D_\phi} \models \phi(\bar X)$. Let $\bar a \in \{0,1,\bot\}^{q+n}$ be a tuple for which 
$$\astruct_{\D_\phi} \, \models \, {\sf MaxRel}(\bar X,\bar a) \, \wedge \, \forall \bar w \forall \bar z\big({\sf MaxComp}(\bar X,\bar w) \wedge (\bar a \sqcup \bar w = \bar z) \, \rightarrow \, \pos(\bar z) \big).$$  Since ${\sf MaxRel}(\bar X,\bar a)$ holds in $\astruct_{\D_\phi}$, it must be the case that $\bar a \in \{\bot\}^q \times \{0,1\}^n$, and hence $\bar a = \bar V$ for some 
$V \subseteq \{x_1,\dots,x_n\}$. We define assignment $\sigma :  \{x_1,\dots,x_n\} \to \{0,1\}$ such that $\sigma(x_i) = 1$ if, and only if, $x_i \in V$. 
Take an arbitrary clause $C_j$, for $j \leq m$. Hence, $\astruct_{\D_\phi} \models \forall \bar z\big({\sf MaxComp}(\bar X,\bar C_j) \wedge (\bar V \sqcup \bar C_j = \bar z) \, \rightarrow \, \pos(\bar z) \big)$. Since $(\bar X,\bar C_j)$ satisfies ${\sf MaxComp}$, 
we obtain that$(\bar C_j,\bar V)$ belongs to the interpretation of $\pos$ in $\astruct_{\D_\phi}$. Hence by definition, there is exactly one variable from $C_j$ in $V$. We conclude that there exists exactly one variable from $C_j$ that is assigned value 1 under $\sigma$. 

%Our proof is based on the classical idea of {\em quantifier elimination}. In particular, we show that there is a computable function that takes a \FO-formula $\phi(\bar x)$ over 
%vocabulary $\sigma = \langle \subseteq,\pos \rangle$, and builds an FO-formula $f(\phi) = \psi(\bar x)$ over an extended vocabulary $\sigma'$ for which the following holds:
%\begin{enumerate}
%\item $\psi$ is quantifier-free, 
%\item for every $n$-ary decision tree $\D$ and tuple $\bar a$ over $\{0,1,\bot\}^n$ of the same arity than $\bar x$, 
%we have that $$(\astruct_\D,\bar a) \models \phi \ \ \Leftrightarrow \ \ (\astruct^{\rm ext}_{D},\bar a) \models \psi,$$ 
%where $\astruct^{\rm ext}_{\D}$ is a structure over $\sigma'$ that depends on $\D$ and $\phi$, and 
%\item checking if $(\astruct_\D^{\rm ext},\bar a) \models \psi$, on input $\D$ and $\bar a$, can be carried out in polynomial time. 
%\end{enumerate}  
%
%We first explain how the vocabulary $\sigma'$ is defined and interpreted in $\astruct^{\rm ext}_{\D}$. Let 
%$x_1,\dots,x_k$ be an enumeration of the variables used in $\phi$. With each $S,T \subseteq \{x_1,\dots,x_k\}$, we associate three new relation symbols
%$\P_{S,T}$, $\N_{S,T}$, $\U_{S,T}$ in $\sigma'$, all of which have the same arity $|S| + |T| + 1$. 
%Such symbols have the following interpretation in $\astruct^{\rm ext}_{\D}$, assuming that $\bar x_S = \{x_1,\dots,x_k\} \cap S$, 
%$\bar x_T = \{x_1,\dots,x_k\} \cap T$, and the formula
%$\alpha(\bar x_S,\bar x_T)$ is defined as $$\bigwedge_{x_i \in S} x_i \subseteq y \, \wedge \, \bigwedge_{x_i \not\in S} x_i \not\subseteq y \, \wedge \, \bigwedge_{x_i \in T} y \subseteq x_i \, \wedge \, \bigwedge_{x_i \not\in T} y \not\subseteq x_i).$$ Then, for arbitrary tuples $\bar a,\bar b$ over $\{0,1,\bot\}^{n}$ with arity $|S|$ and $|T|$, respectively, we have   
%\begin{itemize} 
%\item $(\astruct^{\rm ext}_{\D},\bar a,\bar b) \models \P_{S,T}(\bar x_S,\bar y_S)$ iff $(\astruct_\D,\bar a,\bar b) \, \models \, \exists y (\pos(y) \, \wedge \, \alpha(\bar x_S,\bar x_T,y))$,   
%\item $(\astruct^{\rm ext}_{\D},\bar a,\bar b) \models \N_{S,T}(\bar x_S,\bar y_S)$ iff $(\astruct_\D,\bar a,\bar b) \, \models \, \exists y (\textsc{Full}(y) \wedge \neg\pos(y) \, \wedge \, \alpha(\bar x_S,\bar x_T,y))$, and
%\item $(\astruct^{\rm ext}_{\D},\bar a,\bar b) \models \U_{S,T}(\bar x_S,\bar y_S)$ iff $(\astruct_\D,\bar a,\bar b) \, \models \, \exists y ( \neg \textsc{Full}(y) \wedge \, \alpha(\bar x_S,\bar x_T,y))$.
%\end{itemize} 
%
%We start by observing the following fact, which establishes property (3) for our quantifier elimination procedure. 
%
%\begin{claim} Let $\sigma'$ be the extension of $\sigma$ with respect to variables $\{x_1,\dots,x_k\}$ defined as above. Fix an arbitrary quantifier-free formula 
%$\psi$ over $\sigma'$.  
%Given an $n$-ary decision tree $\D$ and a tuple $\bar a$ over $\{0,1,\bot\}^n$ of the same arity as $\bar x$, 
%checking if $(\astruct^{\rm ext}_{\D},\bar a) \models \psi$ can be carried out in polynomial time. 
%%The same holds for $\N_{S,T}$ and $\U_{S,T}$.  
%\end{claim} 
%
%We now prove the remaining properties of the quantifier elimination procedure. 
%%The proof is inductive. 
%It suffices to show that for each $\phi$ of the form $\exists y \phi_0(\bar x,y)$, where $\phi_0$ is a quantifier-free formula over $\sigma'$, 
%one can build a quantifier-free formula $\psi(\bar x)$ over $\sigma'$ such that, for every $n$-ary decision tree $\D$ and tuple $\bar a$ over $\{0,1,\bot\}^n$ of the same arity than $\bar x$, 
%$$(\astruct_\D,\bar a) \models \phi \ \ \Leftrightarrow \ \ (\astruct^{\rm ext}_{D},\bar a) \models \psi.$$ 
%
%We first define some terminology. An {\em atomic type over $\bar x$} is a set $\cal A$ of formulas satisfying the following. 
%\begin{itemize}
%\item For each $x \in \bar x$, either $\pos(x)$, $\textsc{Full}(x) \wedge \neg {\rm Pos}(x)$, or $\neg \textsc{Full}(x)$ belongs to $\cal A$.
%\item For each ordered pair $(x,y)$ of variables in $\bar x$, either $x \subseteq y$ or $x \not\subseteq y$ belongs to $\cal A$. 
%\end{itemize}  
% 
%


%\newcommand{\enc}{{\rm enc}}  
%Our proof is divided in several steps. 
%
%\paragraph{Structures induced by $\subseteq$.} 
%We start by establishing the following technical lemma which states that if two models have a sufficiently large number of features, then they cannot be distinguished by any $\FO$ formula of a given quantifier depth that uses exclusively the binary predicate $\subseteq$.   
%
%\begin{lemma} \label{lemma:large-types}
%For each $k \geq 0$, if $d,d' \geq 4^k$ then 
%$\langle\{0,1,\bot\}^d,\subseteq \rangle \equiv_k \langle\{0,1,\bot\}^{d'},\subseteq \rangle$. 
%\end{lemma} 
%
%\begin{proof}
%Before proving the lemma we establish some auxiliary results. 
%For a set $Y = \{y_1,\dots,y_d\}$, we use $\bar Y = \{\bar y_1,\dots,\bar y_d\}$ to denote a disjoint copy of it. For $i \leq d$, we call $y_i$ and $\bar y_i$ {\em twins}. 
%If $X,Y,\bar Y$ are pairwise disjoint sets, we write $2^{X;Y}$ to denote the set of all subsets of $X \cup Y \cup \bar Y$. We abuse notation and use $\subseteq$ to denote the containment relation between elements in $2^{X;Y}$ (but keeping in mind that we use the same symbol over $\{0,1,\bot\}^d$ to represent the "completion" relation). 
%
%Consider sets $X_1,X_2,Y_1,Y_2$ and structures of the form $\langle 2^{X_1;Y_1}, \subseteq \rangle$ and 
%  $\langle 2^{X_2;Y_2}, \subseteq \rangle$. We want to study first when these structures are indistinguishable by a restricted version
%  of the EF game defined as follows. In each round the spoiler can only choose an element $A \subseteq X_1 \cup Y_1 \cup \bar Y_1$ 
%  that does not contain twin elements in $Y_1 \cup \bar Y_1$, and the duplicator must respond with an element $B \subseteq X_2 \cup Y_2 \cup \bar Y_2$ 
%  that does not contain twin elements in $Y_2 \cup \bar Y_2$ (or viceversa).  We denote this as $\langle 2^{X_1;Y_1}, \subseteq \rangle \, \equiv_k^r 
%   \, \langle 2^{X_2;Y_2}, \subseteq \rangle$. 
%   
%   \begin{claim} \label{claim:thr} 
%   If $X_1$ and $X_2$ have exactly the same number of elements up to threshold $4^{k}$, and the same holds for 
%   $Y_1$ and $Y_2$, then $\langle 2^{X_1;Y_1}, \subseteq \rangle \, \equiv_k^r 
%   \, \langle 2^{X_2;Y_2}, \subseteq \rangle$. 
%   \end{claim} 
%   
%   \begin{proof}
%   We first observe the following. Fix an arbitrary $k \geq 0$. 
%   Consider 
%pairwise disjoint 
%   sets $X_1,X_2,Y_1,Y_2,Z_1,Z_2,U_1,V_1,U_2,V_2$. Then, if both $\langle 2^{X_1;Y_1 \cup Z_1},\subseteq \rangle \equiv^r_k \langle 2^{X_2;Y_2 \cup Z_2},\subseteq \rangle$ and 
%   $\langle 2^{U_1;V_1},\subseteq \rangle \equiv^r_k \langle 2^{U_2;V_2},\subseteq \rangle$ hold, we can conclude that 
%   \begin{equation*}
%   \langle 2^{X_1 \cup U_1;Y_1 \cup Z_1 \cup V_1},\subseteq,(X_1 \cup Y_1 \cup \bar Z_1) \rangle \ \equiv^r_k \ \langle 2^{X_2 \cup U_2;Y_2 \cup Z_2 \cup V_2},\subseteq,(X_2 \cup Y_2 \cup \bar Z_2)\rangle.
%   \end{equation*}  
%   In fact, a standard composition argument establishes that
%   \begin{equation}
%   \label{eq:games}
%   \langle 2^{X_1 \cup U_1;Y_1 \cup Z_1 \cup V_1},\subseteq \rangle \ \equiv^r_k \ \langle 2^{X_2 \cup U_2;Y_2 \cup Z_2 \cup V_2},\subseteq \rangle;
%     \end{equation} see, e.g., Claim 5.6 in \cite{Lib04}. This idea can be explained as follows. 
%   Each move $A$ by the spoiler over $2^{X_1 \cup U_1;Y_1 \cup Z_1 \cup V_1}$ is split in two parts: $A_1 \in 2^{X_1;Y_1 \cup Z_1}$ and $A_2 \in 2^{U_1;V_1}$. By definition, neither $A_1$ nor $A_2$ contains twin elements. The duplicator then looks at its winning strategy on both games, and finds a response $B_1$ without twin elements in $2^{X_2;Y_2 \cup Z_2}$ and a response $B_2$ without twin elements in $2^{U_2;V_2}$, in such a way that 
%   $\langle 2^{X_1;Y_1 \cup Z_1},\subseteq,A_1 \rangle \equiv^r_{k-1} \langle 2^{X_2;Y_2 \cup Z_2},\subseteq,B_1 \rangle$ and 
%   $\langle 2^{U_1;V_1},\subseteq,A_2 \rangle \equiv^r_{k-1} \langle 2^{U_2;V_2},\subseteq,B_2 \rangle$. 
%   We conclude that 
%   \begin{equation}
%   \label{eq:ind-game}
%   \langle 2^{X_1 \cup U_1;Y_1 \cup Z_1 \cup V_1},\subseteq,A \rangle \ \equiv^r_{k-1} \ \langle 2^{X_2 \cup U_2;Y_2 \cup Z_2 \cup V_2},\subseteq,B \rangle;
%   \end{equation} 
%   Notice that, by definition, $B = B_1 \cup B_2$ contains no twin elements. Hence, for every $A$ over $2^{X_1 \cup U_1;Y_1 \cup Z_1 \cup V_1}$ without twin elements, 
%   there is a $B$ over $2^{X_2 \cup U_2;Y_2 \cup Z_2 \cup V_2}$ without twin elements 
%   for which (\eqref{eq:ind-game}) holds. This is equivalent to saying that (\eqref{eq:games}) holds. 
%   
%  It only remains to show that the game played in this way can also preserve the constants $(X_1 \cup Y_1 \cup \bar Z_1)$ and $(X_2 \cup Y_2 \cup \bar Z_2)$.  
%  For this, it suffices to show that the game on $\langle 2^{X_1;Y_1 \cup Z_1},\subseteq \rangle \equiv^r_k \langle 2^{X_2;Y_2 \cup Z_2},\subseteq \rangle$ can also be assumed to preserve them. In fact, $(X_1 \cup Y_1 \cup \bar Z_1)$ has the property of being maximal among those elements in $2^{X_1; Y_1 \cup Z_1}$ without twin elements.  
%  Hence, if there is at least one round left in the game and spoiler chooses $A = X_1 \cup Y_1 \cup \bar Z_1$, the duplicator must respond with an element $B$ in $2^{X_2; Y_2 \cup Z_2}$
%  that is also maximal among those without twin elements. By symmetry, we can assume without loss of generality that $B = X_2 \cup Y_2 \cup \bar Z_2$. In turn, if there are no further moves in the game and spoiler plays $A$, then the duplicator can safely respond with $B$ without affecting the partial isomorphism.  
%%   Each move $A \subseteq X_1 \cup U_1 \cup Y_1 \cup V_1$ without twin elements played by the spoiler on structure 
%
%%   $A_1 \subseteq X_1$, $B_1 \subseteq Y_1$, $C_1 \subseteq \bar Y_1$, $A_2 \subseteq X_2$,  
%%   $B_2 \subseteq Y_2$, and $C_2 \subseteq \bar Y_2$, where neither $B_1 \cup C_1$ nor $B_2 \cup C_2$ contains twin elements. Let us also 
%%   define $C'_1 = \{y \in Y_1 \mid \bar y \in C_1\}$, $C'_2 = \{y \in Y_2 \mid \bar  y \in C_2\}$, 
%%   %$B'_1 = \{\bar y \in Z_1 \mid \bar y \in B_1\}$,  
%%   %$B'_2 = \{\bar y \in Z_2 \mid \bar y \in B_2\}$, 
%%   $D_1 = \{y \in Y_1 \mid y \not\in B_1,\, y \not\in C_1\}$, and $D_2 = \{y \in Y_2 \mid y \not\in B_2,\, y \not\in C_2\}$. Then, if
%% \begin{itemize} 
%%  \item  
%%   $\langle 2^{A_1; B_1 \cup C'_1},\subseteq \rangle \equiv_k^r \langle 2^{A_2; B_2 \cup C'_2},\subseteq \rangle$, and
%%   \item $\langle 2^{(X_1 \setminus A_1);D_1},\subseteq \rangle \equiv_k^r \langle 2^{(X_2 \setminus A_2);D_2}\rangle$, 
%%   \end{itemize}
%%   we can conclude $\langle 2^{X_1;Y_1},\subseteq,(A_1 \cup B_1 \cup C_1)\rangle \, \equiv_k^r \, \langle 2^{X_2;Y_2},\subseteq,(A_2 \cup B_2 \cup C_2)\rangle$. 
%   
%   We now prove the claim by induction on $k \geq 0$. The cases when $k = 0,1$ are straightforward. For the inductive case for $k+1$ we 
%   only consider the case in which $|X_1|,|X_2|,|Y_1|,|Y_2| \geq 4^{k+1}$, as all other cases can be treated in a similar fashion. 
%   Assume without loss of generality that, for the first round. the spoiler chooses a set  $U \subseteq X_1 \cup Y_1 \cup \bar Y_1$ without twin elements. We define $X_1^U = U \cap X_1$, 
%   $Y_1^U = U \cap Y_1$, and $Z_1^U = U \cap \bar Y_1$. The response of the duplicator will be a set $V = X_2^V \cup Y_2^V \cup Z_2^V$, with $X_2^V = V \cap X_2$, $Y_2^V = V \cap Y_2$, and $Z_2^V = V \cap \bar Y_2$, defined as follows.  
%    
%    \begin{itemize} 
%    
%    \item For defining $X_2^V$ we do the following. 
%   
%    \begin{itemize} 
%    \item If $|X_1^U| < 4^k$, we choose $X_2^V$ to be any subset of $X_2$ with $|X_2^V| = |X_1^U|$. 
%    \item If $|X_1 \setminus X_1^U| < 4^k$, we choose $X_2^V$ to be any subset of $X_2$ for which $|X_1 \setminus X_1^U| = |X_2 \setminus X_2^V|$.
%    \item Otherwise, we choose $X_2^V$ to be any subset of $X_2$ for which  $|X_2^V|, |X_2 \setminus X_2^V| \geq 4^k$. 
%    \end{itemize} 
%    It is easy to see that a $X_2^V$ with the required properties can always be found (as $|X_1|,|X_2| \geq 4^{k+1}$). 
%    Moreover, $X_1^U$ and $X_2^V$ have exactly the same number of elements up to threshold $4^{k}$, and the same holds for 
%   $X_1 \setminus X_1^U$ and $X_2 \setminus X_2^V$.  
%   
%   \item For defining $Y_2^V$ we do the following. 
%   
%   \begin{itemize} 
%    \item If $|Y_1^U| < 2 \cdot 4^k$, we choose $Y_2^V$ to be any subset of $Y_2$ with $|Y_1^U| = |Y_2^V|$. 
%    \item If $|Y_1 \setminus Y_1^U| < 2 \cdot 4^k$, we choose $Y_2^V$ to be any subset of $Y_2$ for which $|Y_1 \setminus Y_1^U| = |Y_2 \setminus Y_2^U|$.
%    \item Otherwise, we choose $Y_2^V$ to be any subset of $Y_2$ for which  $|Y_2^V|, |Y_2 \setminus Y_2^V| \geq 2 \cdot 4^k$. 
%    \end{itemize} 
%    It is easy to see that a $Y_2^V$ with the required properties can always be found (as $|Y_1|,|Y_2| \geq 4^{k+1}$). 
%    Moreover, $Y_1^U$ and $Y_2^V$ have exactly the same number of elements up to threshold $2 \cdot 4^{k}$, and the same holds for 
%   $Y_1 \setminus Y_1^U$ and $Y_2 \setminus Y_2^V$.  
%   
%   \item We now define $Z_2^V$. First, since $U$ contains no twin elements, it must be the case that 
%   $Z_1^U \subseteq M_1 = \{\bar y \in \bar Y_1 \mid y \in Y_1 \setminus Y_1^U\}$. In order to respect the required strategy, the duplicator has to choose 
%   a $Z_2^V \subseteq M_2 = \{\bar y \in \bar Y_2 \mid y \in Y_2 \setminus Y_2^V\}$. But recall from the definition of $Y_2^V$ that 
%   $Y_1 \setminus Y_1^U$ and $Y_2 \setminus Y_2^V$ have exactly the same number of elements up to threshold $2 \cdot 4^{k}$, and thus the same holds for $M_1$ and $M_2$. 
%   We can then proceed as follows. 
%   
%   \begin{itemize} 
%    \item If $|Z_1^U| < 4^k$, we choose $Z_2^V$ to be any subset of $M_2$ with $|Z_1^U| = |Z_2^V|$. 
%    \item If $|M_1 \setminus Z_1^U| < 4^k$, we choose $Z_2^V$ to be any subset of $M_2$ for which $|Z_1 \setminus Z_1^U| = |Z_2 \setminus Z_2^U|$.
%    \item Otherwise, we choose $Z_2^V$ to be any subset of $M_2$ for which  $|Z_2^V|, |M_2 \setminus Z_2^V| \geq 4^k$. 
%    \end{itemize} 
%    It is easy to see that a $Z_2^V$ with the required properties can always be found (as  
%    $M_1$ and $M_2$ have exactly the same number of elements up to threshold $2 \cdot 4^{k}$). 
%    Moreover, $Z_1^U$ and $Z_2^V$ have exactly the same number of elements up to threshold $4^{k}$, and the same holds for 
%   $M_1 \setminus Z_1^U$ and $M_2 \setminus Z_2^V$.  
%   \end{itemize} 
%   
%   Let us now define the following sets: 
%   \begin{equation*} 
%    W_1 \  =   \    \{y \in Y_1 \mid y \not\in Y_1^U,\, \bar y \not\in Z_1^U\}, \ \ \ \ \ \ \ 
%    W_2 \  =  \   \{y \in Y_2 \mid y \not\in Y_2^U,\, \bar y \not\in Z_2^U\}.
%   %, \\
%   %& W_1 \  =  \  & \{y \in Y_1 \mid \bar y \in Z_1^U\}, \ \ \ \ & W_2  =  & \{y \in Y_2 \mid  \bar y \in Z_2^U\}, \\
%   %& \bar W_1 \  =  \  & \{\bar y \in Z_1 \mid y \in Y_1^U\}, \ \ \ \ & \bar W_2  =  & \{\bar y \in Z_2 \mid  y \in Y_2^U\}.
%   \end{equation*} 
%   Recall from our previous observation that $X_1^U$ and $X_2^V$ have exactly the same number of elements up to threshold $4^{k}$, and the same holds for 
%  $Y_1^U$ and $Y_2^V$, $Z_1^U$ and $Z_2^V$, and 
%   $M_1 \setminus Z_1^U$ and $M_2 \setminus Z_2^V$. This implies, in particular, that $W_1$ and $W_2$ 
%  have exactly the same number of elements up to threshold $4^{k}$, since  $|W_1| = |M_1 \setminus Z_1^U|$ and  $|W_2| = |M_1 \setminus Z_2^V|$.
%   By induction hypothesis, we obtain then that 
%   \begin{eqnarray*} \langle 2^{X^U_1; Y_1^U \cup \bar Z_1^U}, \subseteq \rangle \ & \equiv_k^r &
%   \  \langle 2^{X^V_2; Y_2^V \cup \bar Z_2^V}, \subseteq \rangle, \\ 
%   \langle 2^{(X_1 \setminus 
%   X^U_1);W_1}, \subseteq \rangle \ & \equiv_k^r &
%   \ \langle 2^{(X_2 \setminus X^V_2);W_2}, \subseteq \rangle. 
%   \end{eqnarray*} 
%   where $\bar Z_1^U = \{y \in Y_1 \mid \bar y \in Z_1^U\}$ and $\bar Z_2^U = \{y \in Y_2 \mid \bar y \in Z_2^U\}$. 
%   
%   From our previous composition argument, we obtain then that $\langle 2^{X_1;Y_1},\subseteq,U \rangle \equiv^r_{k-1} \langle 2^{X_2;Y_2},\subseteq,V \rangle$. Henceforth, for every $U \subseteq X_1 \cup Y_1 \cup Z_1$ containing no twin elements, there is a 
%   $V \subseteq X_2 \cup Y_2 \cup Z_2$ containing no twin elements for which $\langle 2^{X_1;Y_1},\subseteq,U \rangle \equiv^r_{k-1} \langle 2^{X_2;Y_2},\subseteq,V \rangle$. This is equivalent to 
%   what we aimed to prove, namely, that $\langle 2^{X_1;Y_1},\subseteq \rangle \equiv^r_{k} \langle 2^{X_2;Y_2},\subseteq \rangle$.
%   \end{proof} 
%   
%   We now explain how Lemma \ref{lemma:large-types} follows from Claim \ref{claim:thr}. Fix $d \geq 0$ 
%   and let $X_d = \{x_1,\dots,x_d\}$. We denote by $2^{\emptyset;X_d}_c$ the set of all $A \subseteq X_d \cup \bar X_d$ that contain no twin elements.  
%   Notice that the structures  
%   $\langle \{0,1,\bot\}^d,\subseteq \rangle$ and $\langle 2^{\emptyset;X_d}_c,\subseteq \rangle$ are isomorphic via the mapping 
%   $f : \{0,1,\bot\}^d \to 2^{X_d \cup \bar X_d}$ such that, for each instance $\bar v = (v_1,\dots,v_d) \in \{0,1,\bot\}^d$ and $i \leq d$, 
%   we have that 
%   \begin{itemize} 
%   \item $x_i \in f(\bar v) \, \Leftrightarrow \, v_i = 1$, 
%   \item $\bar x_i \in f(\bar v) \, \Leftrightarrow \, v_i = 0$, and 
%   \item $x_i,\bar x_i \not\in f(\bar v)$, otherwise. 
%   \end{itemize}
%   Take $d,d' \geq 4^k$. We then have that 
%   $$\langle\{0,1,\bot\}^d,\subseteq \rangle \, \equiv_k \, \langle\{0,1,\bot\}^{d'},\subseteq \rangle \ \Longleftrightarrow \  
%   \langle 2_c^{\emptyset;X_d},\subseteq \rangle \, \equiv_k \, \langle 2_c^{\emptyset;X_{d'}},\subseteq \rangle.$$ But the latter is equivalent to 
%   $\langle 2^{\emptyset;X_d},\subseteq \rangle \equiv_k^r \langle 2^{\emptyset;X_{d'}},\subseteq \rangle$. The result then follows from Claim 
%   \ref{claim:thr}. 
%   \end{proof} 
%
%
%\paragraph{Restriction to fully-ordered decision trees.}
%Consider an $n$-ary decision tree $\D = (T,\lambda)$, where $T$ is a binary tree and $\lambda$ is a mapping sending each internal node to a variable in 
%$\{x_1,\dots,x_n\}$ and each leaf to a Boolean value in $\{\true,\false\}$. Recall that each internal node in $\D$ has two outgoing edges: one labeled 0 and the 
%other one labeled 1. We call $\D$ {\em fully-ordered} if $\lambda$ labels each internal node at distance $i$ from the root, for $i \geq 0$, with variable $x_{i+1}$. Notice that each 
%fully-ordered decision tree over $X = \{x_1,\dots,x_n\}$ implicitly assumes an order on the set $X$. We always think of such an order as being $x_1 < x_2 < \ldots < x_n$. 
%
%We show here that for each decision tree $\D = (T,\lambda)$ over $\{x_1,\dots,x_n\}$, 
%there exists a fully-ordered decision tree $\D_{\rm ord} = (T,\lambda')$ such that $\astruct_\D \cong \astruct_{\D_{\rm ord}}$. In particular, 
%the decision tree $\D_{\rm ord}$ is defined over the same tree $T$ as $\D$, but $\lambda'$ labels each internal node at distance $i$ from the root, for $i \geq 0$, with variable $x_{i+1}$. 
%Notice that $\lambda'$ is well-defined as, by definition, decision trees do not repeat variables along a branch, and thus $\D$ only contains internal nodes at depth at most $n-1$ from the root. 
%The labels of the edges and leaves in $\D_{\rm ord}$ are the same than in $\D$.  
%
%\begin{lemma} \label{lemma:iso} 
%It is the case that $\astruct_\D \cong \astruct_{\D_{\rm ord}}$, for every decision tree $\D$. 
%\end{lemma}
%
%\begin{proof} 
%%With each node $t \in T$
%Consider an arbitrary decision tree $\D = (T,\lambda)$ over $\{x_1,\dots,x_n\}$. 
%Every instance $\bar v=(v_1,\ldots,v_n)\in \{0,1,\bot\}^n$ defines a unique path $\pi(\D,\bar v)$ from the root to a node in $T$ in terms of $\D$.  
%This path satisfies the following condition, until it fails or it reaches a leaf: for every non-leaf node~$u$ in~$\pi(\D,\bar v)$, if~$i$ is the label of~$u$ in $\D$ and $v_i \in \{0,1\}$, for $i \leq n$, 
%then the path~$\pi(\D,\bar v)$ goes through the edge that is labeled with~$v_i$ in $\D$. The procedure fails if it finds an internal node labeled $i$ for which $v_i = \bot$. 
%
%We define a mapping $f : \{0,1,\bot\}^n \to \{0,1,\bot\}^n$ as follows. Take an arbitrary $\bar v=(v_1,\ldots,v_n)\in \{0,1,\bot\}^n$ and suppose that the 
%node labels of the path $\pi(\D,\bar v)$ are ${i_1} \cdots {i_\ell}$, for $1 \leq i_1,\dots,i_\ell \leq n$. We define $f(\bar v)$ to be the tuple which is obtained 
%from $\bar v$ by interchanging the values $v_j$ and $v_{i_j}$, for each $j \leq \ell$. For instance, if the labels of the path are 3 and 4, and $\bar v = (\bot,0,1,0)$, then 
%$f(\bar v) = (1,0,\bot,0)$. We claim that $f$ is a bijection.  
%
%We finish by observing that $f$ is an isomorphism between 
%$\astruct_\D$ and $\astruct_{\D_{\rm ord}}$. Since $f$ is a bijection, it only remains to show that for every $\bar u,\bar v \in \{0,1,\bot\}^n$ we have that 
%$\bar u \subseteq \bar v$ holds in $\D$ iff $f(\bar u) \subseteq f(\bar v)$ holds in $\D_{\rm ord}$. But this is clear from the fact that 
%
%%is the label 
%%of the nodes   
%%
%%For a node $t \in T$, we write ${\sf cons}(\D,t)$ for the set of instances $\bar v=(v_1,\ldots,v_n)\in \{0,1,\bot\}^n$ for which the path $\pi(\D,\bar v)$ finishes in node $t$.  
%%
%%For $S \subseteq \{x_1,\dots,x_n\}$ and $\bar v=(v_1,\ldots,v_n)\in \{0,1,\bot\}^n$, 
%%we write $\bar v_{|S}$ for the restriction of $\bar v$ to the variables in $S$.
%%The isomorphism witnessing $\astruct_\D \cong \astruct_{\D_{\rm ord}}$ maps instances in ${\sf cons}(\D,t)$, for $t \in T$, to 
%%instances in ${\sf cons}(\D_{\rm ord},t)$. It is constructed as follows. 
%%Fix a node $t \in T$. Let us denote by ${\sf Undef}(\D,t)$ the set of all variables $x_i$, for $i \leq n$, such that 
%%no proper ancestor of $t$ in $\D$ is labeled $i$.  It is clear that $\bar u_{|{\sf undef}(\D,t)} = \bar v_{|{\sf undef}(\D,t)}$, 
%%for every $t \in T$ and $\bar u,\bar v \in {\sf Cons}(\D,t)$, and the same holds over $\D_{\rm ord}$. 
%%%For an instance $\bar v \in {\sf cons}(\D,t)$, we write $\bar v_\downarrow$ for the restriction of $\bar v$ to those 
%%%variables in ${\sf Undef}(\D,t)$, and write 
%%%$\bar v_\uparrow$ for the restriction of $\bar v$ 
%%%formed by the remaining variables.  
%%Moreover, it is not hard to see that 
%%%$|{\sf Undef}(\D,t)| = |{\sf Undef}(\D_{\rm ord},t)|$, it holds that $\bar v^\uparrow = \bar u^\uparrow$, for every pair $\bar v,\bar u \in {\sf cons}(\D,t)$, and 
%%there is a 
%%bijection $g_t :  {\sf Cons}(\D,t) \to {\sf Cons}(\D_{\rm ord},t)$ and a permutation $\rho_t$ over ${\sf Undef}(\D_{\rm ord},t)$, 
%%with 
%%$$\bar v_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D,t)} \ = \ \rho_t(g_t(\bar v)_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D_{\rm ord},t)}), \text{ for each $\bar v \in \{0,1,\bot\}^n \cap {\sf cons}(\D,t)$.}$$
%%Here, $\rho_t(\bar u)$ is the tuple which is obtained from $\bar u$ by applying the permutation $\rho$ on the components in ${\sf Undef}(\D_{\rm ord},t)$. 
%%%We denote by $h_t$ the mapping that sends each element $\bar v \in {\sf cons}(\D,t)$ to the unique element $\bar u \in {\sf cons}(\D_{\rm ord},t)$ with 
%%%$\bar u_\downarrow = g_t(\bar v_\downarrow)$. 
%%
%%%$$\{\bar v_\downarrow \, \mid \, \bar v \in {\sf cons}(\D,t)\} \ = \ \{g_t(\bar v_\downarrow) \, \mid \, \bar v \in {\sf cons}(\D_{\rm ord},t)\}.$$ 
%%
%%We can then define a bijection $f : \{0,1,\bot\}^n \to \{0,1,\bot\}^n$ satisfying $f(\bar v) = g_t(\bar v)$,  for each 
%%$\bar v = (v_1,\dots,v_n) \in \{0,1,\bot\}^n$ with $\bar v \in {\sf cons}(\D,t)$. We show next that $f$ is an isomorphism between 
%%$\astruct_\D$ and $\astruct_{\D_{\rm ord}}$. Since $f$ is a bijection, it remains to show that for every $\bar u,\bar v \in \{0,1,\bot\}^n$ we have that 
%%$\bar u \subseteq \bar v$ holds in $\D$ iff $f(\bar u) \subseteq f(\bar v)$ holds in $\D_{\rm ord}$. Suppose first that $\bar u \subseteq \bar v$ holds in $\D$. 
%%We only have to consider two cases since $\bar u \subseteq \bar v$ implies $\bar u \in {\sf cons}(\D,t)$ and $\bar v \in {\sf cons}(\D,t')$, for some $t,t' \in T$ such that $t$ is an ancestor of $t'$.  
%%\begin{itemize}
%%\item
%%The first case is when $\bar u,\bar v \in {\sf cons}(\D,t)$, for some $t \in T$. 
%%Then, by definition, $f(\bar u)_{|{\sf undef}(\D_{\rm ord},t)} = f(\bar v)_{|{\sf undef}(\D_{\rm ord},t)}$. 
%%Moreover, \begin{eqnarray*} 
%%f(\bar u)_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D_{\rm ord},t)} \ = \ \rho_t^{-1}(\bar u_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D,t)}), \\ f(\bar v)_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D_{\rm ord},t)} \ = \ \rho^{-1}_t(\bar v_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D,t)}).
%%\end{eqnarray*}
%%We conclude that $f(\bar u) \subseteq f(\bar v)$ holds in $\D_{\rm ord}$ since $\bar u_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D,t)} \subseteq \bar v_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D,t)}$ holds in $\D$. 
%%\item The second case is when $\bar u \in {\sf cons}(\D,t)$ and $\bar v \in {\sf cons}(\D,t')$, for nodes $t,t' \in T$ with $t'$ a proper descendant of $t$. 
%%Let ${\sf Common}(\D,t,t')$ be the set of variables $x_i \in \{x_1,\dots,x_n\}$ such that some node $t'' \in T$ that is a descendant of $t$, but a proper ancestor of $t'$, is labeled $i$.  
%%We observe the following facts: 
%%\begin{itemize}
%%\item $f(\bar u)_{|{\sf undef}(\D_{\rm ord},t)} = f(\bar v)_{|{\sf undef}(\D_{\rm ord},t)}$, 
%%\item $f(\bar u)_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D_{\rm ord},t')} \ = \ \rho_{t'}^{-1}(\bar u_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D,t')})$, 
%%\item $f(\bar v)_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D_{\rm ord},t')} \ = \ \rho_{t'}^{-1}(\bar v_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D,t')})$, and 
%%\end{itemize} 
%%We conclude that 
%%\end{itemize}
%%Suppose, in turn, that $\bar u \subseteq \bar v$ does not hold in $\D$. We only have to consider two cases. 
%%\begin{itemize}
%%\item
%%The first case is when $\bar u,\bar v \in {\sf cons}(\D,t)$, for some $t \in T$. 
%%Again, by definition, $f(\bar u)_{|{\sf undef}(\D_{\rm ord},t)} = f(\bar v)_{|{\sf undef}(\D,t)}$. 
%%Moreover, \begin{eqnarray*} 
%%f(\bar u)_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D_{\rm ord},t)} \ = \ \rho^{-1}(\bar u_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D,t)}), \\ f(\bar v)_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D_{\rm ord},t)} \ = \ \rho^{-1}(\bar v_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D,t)}).
%%\end{eqnarray*}
%%We conclude that $f(\bar u) \not\subseteq f(\bar v)$ holds in $\D_{\rm ord}$ since $\bar u_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D,t)} \not\subseteq \bar v_{|\{x_1,\dots,x_n\} \setminus {\sf Undef}(\D,t)}$ holds in $\D$. 
%%
%%%Again, the restrictions of $f(\bar u)$ and $f(\bar v)$ to the variables {\em not} in ${\sf Undef}(\D_{\rm ord},t)$ 
%%%coincide, and the restrictions of $f(\bar u)$ and $f(\bar v)$ to the variables in ${\sf Undef}(\D_{\rm ord},t)$ 
%%%coincide with $\rho^{-1}(\bar u)$ and $\rho^{-1}(\bar v)$, respectively.  
%%%We conclude that $f(\bar u) \subseteq f(\bar v)$ does not in $\D_{\rm ord}$. 
%%\item The second case is when $\bar u \in {\sf Cons}(\D,t)$ and $\bar v \in {\sf Cons}(\D,t')$, for $t'$ not a proper descendant of $t$ in 
%%$\D$.  By definition, then, $f(\bar u) \in {\sf Cons}(\D_{\rm ord},t)$ and $f(\bar v) \in {\sf Cons}(\D_{\rm ord},t')$, which implies that 
%%$f(\bar u) \subseteq f(\bar v)$ does not hold in $\D_{\rm ord}$. 
%%\end{itemize}
%\end{proof} 
%
%Notice, further, that $\D_{\rm ord}$ can be constructed in polynomial time from $\D$. 
%          
%  \paragraph{Encoding of fully-ordered decision trees.}         
%We explain how we encode fully-ordered decision trees as ordered binary trees, 
%with nodes labeled over a finite alphabet that depends only on the quantifier depth $k$ of $\phi$. 
%%A {\em $\Sigma$-labeled ordered binary tree}, for $\Sigma$ a finite alphabet, 
%%is a structure $\cal T$ over the vocabulary that consists of binary relations $\preceq_{\rm left}$ and $\preceq_{\rm right}$, and unary predicates $P_a$ for each 
%%$a \in \Sigma$.  The domain $U$ of $\cal T$ consists of a prefix closed finite subset of $\{0,1\}^*$ that satisfies the following for every $\bar w \in \{0,1\}^*$: 
%%if $\bar w 1 \in U$ then $\bar w 0 \in U$. The interpretation of $\preceq_0$ in $\cal T$ contains all pairs $(\bar w,\bar w0)$, for $\bar w,\bar w0 \in U$, and the 
%%interpretation of $\preceq_1$ in $\cal T$ contains all pairs $(\bar w,\bar w1)$, for $\bar w,\bar w1 \in U$. Finally, the interpretation of the $P_a$s, for $a \in \Sigma$, defines a partition of $U$; that is, each element in $U$ belongs to exactly one set in $(P_a^{\cal T})_{a \in \Sigma}$. 
%Consider a fully-ordered decision tree $\D = (T,\lambda)$ over $\{x_1,\dots,x_n\}$. 
%We build a $\Sigma_k$-ordered binary tree $\enc(\D)$ from $\D$, for $\Sigma_k = \{0,1,\ldots,4^k\}$, 
%in the following way. The domain of $\enc(\D)$ is the set of all assignments for $(x_1,\dots,x_i)$ over $\{0,1\}$, for each 
%$i \leq n$, that are consistent with some path in $\D$ that goes from the root of $T$ to some node at depth $i$.  
%The interpretation of $P_j$ in $\enc(\D)$, for $j \in \{0,1,\ldots,4^k\}$, is defined as follows: 
%$$P_j^{\enc(\D)} \ = \ 
%\begin{cases} 
%\{t \mid \text{depth of $t$ in $T$ is $\ell$ and $n - \ell = j$}\}, \ \ \ & \text{if $j < 4^k$}, \\ 
%\{t \mid \text{depth of $t$ in $T$ is $\ell$ and $n - \ell \geq 4^k$}\}, & \text{if $j = 4^k$}. 
%\end{cases} 
%$$ 
%
%We now establish the following key lemma, which establishes that $\equiv_k$-indistinguishability for fully-ordered decision trees can be 
%checked at the level of their encodings.        
%
%\begin{lemma} \label{lemma:ind} 
%Let $\D$ and $\D'$ be fully ordered decision trees. For every $k \geq 0$, we have that 
%$$\astruct_\D \, \equiv_k \, \astruct_{\D'} \ \ \Longleftrightarrow \ \ \enc(\D) \equiv_k \enc(\D').$$ 
%\end{lemma}
%
%\begin{proof}xx
%\end{proof}
%
%Observe that $\enc(\D)$, for $\D$ a fully-ordered decision tree, can be constructed in polynomial time in the size of $\D$ (as the size of $\Sigma_k$ is fixed, and we can check for each 
%node in polynomial time what its label in $\Sigma_k$ is). 
%
%\paragraph{Recognizing encodings with tree automata.} Not every $\Sigma_k$-labeled ordered binary tree represents the encoding of a fully-ordered decision tree. 
%For instance, encodings of fully-ordered decision trees always satisfy that a node labeled $P_2$ can only have children labeled $P_1$.  Importantly, the set of these encodings is regular, 
%as established next. 
%
%\begin{lemma} \label{lemma:enc} 
%There is a tree automata $\cal A_{\rm enc}$ running on $\Sigma_k$-ordered binary trees that recognizes precisely those structures of the form $\enc(\D)$, for $\D$ a fully-ordered decision tree. Moreover, $\cal A_{\rm enc}$ can be constructed in constructed in constant time (assuming $k$ to be fixed). 
%\end{lemma}
%
%\begin{proof}
%xx
%\end{proof}
%
%Notice that 
%
%\paragraph{From encoding to fully-ordered decision trees.} We observe that fully-ordered decision trees can be recovered in polynomial time from the encodings that represent them.  
%
%\begin{lemma} \label{lemma:recovery} 
%There is a polynomial time procedure that takes a $\Sigma_k$-ordered binary tree $\cal T$ which is accepted by $\cal A_{\rm enc}$, and computes a fully-ordered decision tree 
%$\D$ with $\enc(\D) \cong \cal T$. 
%\end{lemma}
%
%\paragraph{Recognizing types with tree automata.} 
%Let $\Gamma_k$ be the set of all rank-$k$ types of $\Sigma_k$-labeled binary trees. A well-known construction establishes that one can build a 
%deterministic tree automata $\cal A_{\rm types}$ (without final states) running on $\Sigma_k$-ordered binary trees for which the following statements hold: 
%\begin{itemize}
%\item The set of states of $\cal A_{\rm types}$ is $\Gamma_k$, and 
%\item for each $\Sigma_k$-labeled ordered binary tree $\cal T$, the unique run of $\cal A_{\rm types}$ on $\cal T$ labels its root 
%with state $\gamma \in \Gamma$ iff 
%the rank-$k$ type of $\cal T$ is $\gamma$.
%\end{itemize}
%The time that it takes to build this tree automata, although $k$-fold exponential, is still constant for our purposes as $k$, the quantifier depth of $\phi$, is fixed. 
%%In the following, we assume that $g(k)$ is the time that it takes to construct $\cal A_{\rm types}$, for $g : \mathbb{N} \to \mathbb{N}$ a computable function.  
%
%For each $\gamma \in \Gamma$, we denote by $\cal A_\gamma$ the tree automata which is obtained from $\cal A_{\rm types}$ by setting $\gamma$ to be the unique 
%final state. This tree automata, which can be constructed in constant time, accepts precisely those $\Sigma_k$-labeled binary trees whose rank-$k$ type is $\gamma$. 
%
%\paragraph{Polynomial-time evaluation procedure.} We can finally explain the details of our polynomial time procedure. 
%We are given a decision tree $\D = (T,\lambda)$ over $\{x_1,\dots,x_n\}$.
%
%\begin{itemize}
%
%\item 
%We start by building $\D_{\rm ord}$, and then $\enc(\D_{\rm ord})$. This can all be done in polynomial time in the size of the input $\D$ as explained above. 
%
%\item 
%We then run $\cal A_{\rm types}$ on $\enc(\D_{\rm ord})$, which again can be carried out in polynomial time. Let us assume that this run tells us that 
%the rank-$k$ type of $\enc(\D_{\rm ord})$ is $\gamma \in \Gamma$. 
%
%\item We build in constant time a tree automata $\cal A_{\rm enc} \cap \cal A_\gamma$, which accepts precisely those $\Sigma_k$-labeled binary trees  of 
%rank-$k$ type $\gamma$ which represent the 
%encoding of a fully-ordered decision tree. We observe that the language accepted by this tree automata is nonempty, as 
%$\enc(\D_{\rm ord})$ belongs to it. 
%
%\item Since the language of $\cal A_{\rm enc} \cap \cal A_\gamma$ is nonempty, as mentioned above we can build in constant time a $\Sigma_k$-labeled binary 
%tree $\cal T$ that is accepted by it. By definition, $\cal T$ has rank-$k$ type $\gamma$.
%
%\item Given that $\cal T$ is accepted by $\cal A_{\rm enc}$, Lemma \ref{lemma:recovery} tells us that 
%we can construct in polynomial time a fully-ordered decision tree $\D'$ with $\enc(\D') \equiv_k \cal T$.  
%
%\item We finally construct $\astruct_{\D'}$ and evaluate $\phi$ on it. This can all be done in constant time in the size of $\D'$.   
%
%\end{itemize} 
%
%The correctness of the algorithm is ensured by the following line of reasoning:
%\begin{eqnarray*} 
%\astruct_{\D} \ \cong \ \astruct_{\D_{\rm ord}} \ \equiv_k \ \astruct_{\D'}.
%\end{eqnarray*}  
%In fact, $\astruct_{\D} \cong \astruct_{\D_{\rm ord}}$ from Lemma \ref{lemma:iso}. In addition, $\astruct_{\D_{\rm ord}} \equiv_k \astruct_{\D'}$ from Lemma \ref{lemma:ind} since $\enc(\D_{\rm ord}) \equiv_k \cal T$ and $\cal T \equiv_k \enc(\D')$. 

==> the_language.tex <==

%Define First-Order Interpretability Logic (\foil). This is just a first name for the logic, we need the acronym to refer to it.

\subsection{Logical structure for interpretability}

Fix an integer $d$, representing the dimension of \emph{models} (i.e., mappings $\{0, 1\}^d \to \{0, 1\}$) to interpret. Consider then a vocabulary $\sigma_d$ consisting of $3^d$ constant symbols, a unary predicate $\pos(\cdot)$ and a binary predicate $\subseteq(\cdot, \cdot)$, for which we will use infix notation from now on. 

All $\sigma_d$-structures we will consider share a common universe, namely the set $\{0,1, \bot\}^d$, representing the possible instances a $d$-dimensional model could get, with $\bot$ representing a component whose value is undefined. The interpretation of the constants and the $\subseteq(\cdot, \cdot)$ predicate is also shared for all $\sigma_d$-structures. Each of the $3^d$ constants corresponds to a vector of the universe $\{0, 1, \bot\}^d$, and the predicate $\subseteq(\cdot, \cdot)$ is interpreted as
\[
	 x \subseteq y \quad \text{ iff } \quad \left( \bigwedge_{i=1}^d x_i \neq \bot \implies x_i = y_i \right)
\]

For example, it holds that \( \begin{pmatrix}
		0 & \bot & 1 & \bot
	\end{pmatrix} \subseteq \begin{pmatrix}
	0 & 1 & 1 & 0 	
 \end{pmatrix}
\); \\		
but \( \begin{pmatrix}
		0 & \bot & 1 & \bot
	\end{pmatrix} \not\subseteq \begin{pmatrix}
	1 & 1 & \bot & 0 	
 \end{pmatrix}
\).



Given a model $\M$ of dimension $d$, we can associate to it a $\sigma_d$-structure, denoted $\astruct_\M$, which differs from the others $\sigma_d$-structures in its interpretation of the predicate $\pos$. Namely, its interpretation corresponds to all vectors $x \in \{0, 1\}^d$ such that $\M(x) = 1$.

For example, over a model $\M$ of dimension 4, the sentence 
\[
	\phi \coloneqq \exists x \Big( \pos(x) \land \begin{pmatrix}
		0 & 1 & \bot & \bot
	\end{pmatrix} \subseteq x  \Big)
\]
is expressing that $\M$ accepts at least one instance with $0$ in its first component and $1$ in its second.

Note that the size of the structure $\astruct_\M$is too large with respect to the model, i.e., $|\astruct_\M| = \Omega(3^{|\M|})$, and thus we cannot afford to build $\astruct_M$. Instead, we will evaluate formulas on-the-fly.

